Improved Techniques for Quantizing Deep Networks with Adaptive Bit-Widths

Quantizing deep networks with adaptive bit-widths is a promising technique for efficient inference across many devices and resource constraints. In contrast to static methods that repeat the quantization process and train different models for different constraints, adaptive quantization enables us to flexibly adjust the bit-widths of a single deep network during inference for instant adaptation in different scenarios. While existing research shows encouraging results on common image classification benchmarks, this paper investigates how to train such adaptive networks more effectively. Specifically, we present two novel techniques for quantizing deep neural networks with adaptive bit-widths of weights and activations. First, we propose a collaborative strategy to choose a high-precision teacher for transferring knowledge to the low-precision student while jointly optimizing the model with all bit-widths. Second, to effectively transfer knowledge, we develop a dynamic block swapping method by randomly replacing the blocks in the lower-precision student network with the corresponding blocks in the higher-precision teacher network. Extensive experiments on multiple image classification datasets including video classification benchmarks for the first time, well demonstrate the efficacy of our approach over state-of-the-art methods.

==> A5_progressive.tex <==
\section{Progressive Training}
\input{tables/progressive_training}
In the main paper,  we progressively train a quantized model with multiple bit-widths in a descending order (\textit{i.e.}, from 8 bits to 2 bits by sequentially finetuning). In this section, instead, we progressively train a quantized model with multiple bit-widths in a ascending order (\textit{i.e.}, from 2 bits to 8 bits by sequentially finetuning). We compare \ours with two progressive methods in Table~\ref{table:cifar10_resnet18_progressive}. Both progressive training methods experience the performance drop in the bit-width which is trained earlier, i.e. 8 bit in the descending order and 2 bit in the ascending order. \ours with joint training achieves good performance in all precisions. 

==> A6_different_combination.tex <==
\section{Different Bit-width Combinations}
\input{tables/different_B_others}
In this section, we compare all-at-once networks trained with different pre-defined bit-width sets $\mathcal{B}$: namely $\mathcal{B}= \{8, 6, 4, 2\}$, $\mathcal{B}= \{8, 2\}$ and $\mathcal{B}= \{8, 4\}$. We evaluate each network with bit-widths from 2 to 8 bit. If the evaluated bit-width is missing from $\mathcal{B}$, we report its zero-shot testing result. From Table~\ref{table:different_B_others}, we have the following observations. (1) If a network is trained under fewer bit-widths, the performance for the bit-width in $\mathcal{B}$ improves since it is easier for the network to handle fewer bit-widths during the training. (2) When a network is trained with $\mathcal{B} = \{8, 4\}$, 8-bit performance is much better than the one trained with $\mathcal{B} = \{8, 2\}$. It is because training with 4 bit is a closer task to training with 8 bit than training with 2 bit, which results in more positive transferring in the joint training. (3) When a network is trained with $\mathcal{B} = \{8, 6, 4, 2\}$, the middle-precisions achieve higher top-1 accuracy compared with the network trained with $\mathcal{B} = \{8, 2\}$, since the network is unable to keep the good performance for the middle precisions when the supervisions of all middle precisions are missing in $\mathcal{B}$. (4) 2 bit performance drops dramatically when the network is trained 8 and 4 bit. It is important to keep the lowest precision in $\mathcal{B}$ to achieve good performance for it.

==> tables/different_B_others.tex <==
\begin{table}
  \begin{center}
        \resizebox{0.68\linewidth}{!}{
        \begin{tabular}{c|c c c}
            \Xhline{3\arrayrulewidth} 
            $\mathcal{B}$ & $\{8, 6, 4, 2\}$ & $\{8, 2\}$ & $\{8, 4\}$ \\
            \Xhline{3\arrayrulewidth} 
            8-bit & 95.2 &  95.2 &  95.6 \\
            7-bit & 95.2 & 95.2 & 95.5 \\
            6-bit & 95.4 & 95.2 & 95.5 \\
            5-bit & 95.3 & 95.2 & 95.3 \\
            4-bit & 95.1 & 94.5 & 95.5  \\
            3-bit & 94.6 & 94.7 & 93.8 \\
            2-bit & 94.1 & 94.5 & 73.2\\
            \Xhline{3\arrayrulewidth} 
        \end{tabular}}
        \caption{\small\textbf{Evaluation Results on 2 to 8 bits with different $\mathcal{B}$.} On CIFAR10, We train all-at-once quantization network with different pre-defined bit-width sets $\mathcal{B}$ and evaluate with 2 bit to 8 bit. We use zero-shot testing for all missing bit-widths.  }~\label{table:different_B_others}
    \end{center}
    \vspace{-30pt}
\end{table}

==> tables/progressive_training.tex <==
\begin{table}
  \begin{center}
        \resizebox{0.96\linewidth}{!}{
        \begin{tabular}{c|c c c c | c}
            \Xhline{3\arrayrulewidth} 
            Methods & 8-bit & 6-bit & 4-bit & 2-bit &\cellcolor{Gray} $\Delta_\mathcal{B}$ $\uparrow$ \\
            \Xhline{3\arrayrulewidth} 
            Progressive (Descend) & 91.8 & 91.9 & 92.02 & 92.9 & \cellcolor{Gray} 97.1 \\
            Progressive (Ascend) & 94.7 & 94.5 & 94.2 & 87.0 & \cellcolor{Gray} 97.6 \\
             \hline
            \ours (Ours) & 95.2 & 95.4 & 95.1 & 94.1 &\cellcolor{Gray} \textbf{100.1}\\
            \Xhline{3\arrayrulewidth} 
        \end{tabular}} 
        \caption{\small \textbf{Comparison with Progressive Training (Both Ascending and Descending) using ResNet18 on CIFAR10.} }~\label{table:cifar10_resnet18_progressive}
    \end{center}
        \vspace{-20pt}

\end{table}
